Piracy Resistant Watermarks for Deep Neural Networks

As companies continue to invest heavily in larger, more accurate and more robust deep learning models, they are exploring approaches to monetize their models while protecting their intellectual property. Model licensing is promising, but requires a robust tool for owners to claim ownership of models, i.e. a watermark. Unfortunately, current designs have not been able to address piracy attacks, where third parties falsely claim model ownership by embedding their own "pirate watermarks" into an already-watermarked model. We observe that resistance to piracy attacks is fundamentally at odds with the current use of incremental training to embed watermarks into models. In this work, we propose null embedding, a new way to build piracy-resistant watermarks into DNNs that can only take place at a model's initial training. A null embedding takes a bit string (watermark value) as input, and builds strong dependencies between the model's normal classification accuracy and the watermark. As a result, attackers cannot remove an embedded watermark via tuning or incremental training, and cannot add new pirate watermarks to already watermarked models. We empirically show that our proposed watermarks achieve piracy resistance and other watermark properties, over a wide range of tasks and models. Finally, we explore a number of adaptive counter-measures, and show our watermark remains robust against a variety of model modifications, including model fine-tuning, compression, and existing methods to detect/remove backdoors. Our watermarked models are also amenable to transfer learning without losing their watermark properties.

==> Makefile <==
LATEX=latex

BIBTEX=bibtex
BIBFILE=zhao.bib watermark.bib
PAPER=watermark

TEXFILES = watermark.tex \
	intro.tex \
	back.tex \
	threat.tex \
	intuition.tex \
	weakness.tex \
	overview.tex \
	shortanalysis.tex \
	ownership.tex \
	countermeasure.tex \
	eval1.tex \
	transfer.tex \
	discussion.tex \
	appendix.tex \
	revision_appendix.tex \
	response_appendix.tex \


EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

#$(PAPER).pdf: $(PAPER).dvi
#	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> eval.tex <==
\section{Experimental Evaluation}
\label{sec:eval}
In this section, we use empirical experiments on five classification tasks to
validate our proposed watermark design.

%fulfills the requirements listed in
%Section~\ref{sec:requirements}.

\begin{table*}[t]
  \centering
  \resizebox{0.85\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
Task                                                                     & Dataset       & \# Classes & \begin{tabular}[l]{@{}l@{}}Training\\ data size\end{tabular} & \begin{tabular}[l]{@{}l@{}}Test data \\size\end{tabular} & Input size  & Model architecture         \\ \hline
\begin{tabular}[l]{@{}l@{}}Digit Recognition (\mnist)\end{tabular}        & MNIST         & 10       & 60,000                                                     & 10,000                                                 & (28, 28, 1) & 2 Conv + 2 Dense           \\ \hline
\begin{tabular}[l]{@{}l@{}}Traffic Sign Recognition (\gtsrb)\end{tabular} & GTSRB         & 43       & 39,209                                                     & 12,630                                                 & (48, 48, 3) & 6 Conv + 3 Dense           \\ \hline
\begin{tabular}[l]{@{}l@{}}Face Recognition (\youtubeface)\end{tabular}   & \begin{tabular}[l]{@{}l@{}} YouTube Faces\end{tabular} & 1283     & 375,645                                                    & 64,150                                                 &
   (55, 47, 3) & \begin{tabular}[l]{@{}l@{}} 4 Conv + 1 Merge + 1 Dense \end{tabular} \\ \hline
\begin{tabular}[l]{@{}l@{}}Object Recognition 1 (\cifars)\end{tabular}       & CIFAR-10      & 10       & 50,000                                                    &10,000                                                 & (32, 32, 3) & 6 Conv + 3 Dense           \\ \hline
\begin{tabular}[l]{@{}l@{}}Object Recognition 2 (\cifarl)\end{tabular}       & CIFAR-10      & 10       & 50,000                                                    &10,000                                                 & (32, 32, 3) & 21 Conv + 1 Dense           \\ \hline

\end{tabular}
}
\vspace{-.1in}
\caption{Overview of classification tasks with their associated
  datasets and DNN models}
\label{table:dataset}
\vspace{-.1in}
\end{table*}



\subsection{Experimental Setup}
\label{sec:expr_setup}
We use five classification tasks to evaluate
our proposed
ownership watermark design.
%: (1) Digit Recognition (\mnist), %(2) Object Recognition (\cifar),%
%(2) Traffic Sign Recognition (\gtsrb), (3) Face Recognition (\youtubeface),
%(4) Object Recognition (\cifar).
These tasks
use different model architectures and target disjoint types of objects,
allowing us to evaluate our design in a broad array
of settings. We describe each task, its associated dataset and model below, and summarize the details in Table~\ref{table:dataset}.
More details on model structures (Tables~\ref{table:mnist_model}-\ref{table:cifar10_resnet20})
%\ref{table:gtsrb_model}, \ref{table:youtube_model},
%\ref{table:cifar10_small_model}, \ref{table:cifar10_resnet20}),
and
training hyperparameters (Table~\ref{table:params}) as listed in
the Appendix.  For all five tasks, we normalize the pixel value of input images to be
in the range of $[0,1]$.

%such as learning rate, decay, batch size, optimizer type and
%epochs for each task are listed in Table~\ref{table:params} in the appendix.

\begin{packed_itemize}
\item {Digit Recognition} (\mnist~\cite{lecun1998gradient}) is to
  classify images of handwritten digits to one of 10 classes. Each input image
  is normalized so the digit appears in the center.   The
  corresponding classification model contains two convolutional layers and
    two dense layers.

 % Images of the digits have been normalized and centered in a
 %   fixed-size image. We use a model with two convolutional layers and
 %   two dense layers to perform this task.

%  \item {\em Digit Recognition} (\mnist~\cite{lecun1998gradient}). The
 %   task is to classify handwritten digits to one of 10 classes.
  %  Images of the digits have been normalized and centered in a
   % fixed-size image. We use a model with two convolutional layers and
    %two dense layers to perform this task.


\item {Traffic Sign Recognition} (\gtsrb~\cite{Stallkamp2012}) is to recognize 43 types of German
  traffic signs based on the German Traffic Sign
  Benchmark (GTSRB).  The classification model contains six
  convolutional layers and three dense layers.


  % The German Traffic Sign
  % Benchmark (GTSRB) is a multi-class, single-image classification
  % challenge. The task is to correctly recognize 43 different types of
  % German stop signs. We use use a model with six
  % convolutional layers and three dense layers for this task.


\item {Face Recognition} (\youtubeface~\cite{parkhi2015deep,
    schroff2015facenet}) seeks to accurately recognize each individual
  face of $1,284$ people, whose faces are drawn from $3,425$ YouTube
  videos.   Each person in the target dataset  has at least 100 labeled
  images, and their faces are aligned.  The corresponding face
  recognition model is the DeepID model proposed by~\cite{sun2014deep}.
  % This task involves correctly recognizing the
  % faces of $1,284$ people. Data for this task is drawn from $3,425$
  % YouTube videos. All faces included in video frames are aligned, and a label is assigned to each video
  % frame.  We apply preprocessing to filter out labels associated
  % with fewer than $100$ input images (as in prior literature~\cite{wang2019neural}). %Result is a dataset with $1,283$ classes.
  % We use the DeepID model~\cite{sun2014deep} for this task.

\item {Object Recognition 1} (\cifars~\cite{krizhevsky2009learning})
  is to recognize objects on an image as one of the ten object
  types. This task uses the CIFAR-10 dataset with $60000$ color images in $10$
  classes ($6000$ images per class).  Similarly to \gtsrb, the model has six
  convolutional layers and three dense layers.


  % The CIFAR-10 dataset is used
  % to train DNN models to recognize objects in one of $10$ output
  % classes. The dataset consists of $60000$ color images in $10$
  % classes ($6000$ images per class). Similarly to \gtsrb, we use a model with six
  % convolutional layers and three dense layers for this task.

\item {Object Recognition 2} (\cifarl~\cite{krizhevsky2009learning})
  has the same task of recognizing objects as one of the ten object
  types. It uses the same dataset as \cifars but a different DNN model
  architecture, {\em i.e.\/} the ResNet20
  architecture~\cite{he2016deep}, a significantly larger deep neural network,
%This task uses the same
 % dataset as \cifars. However, we use ResNet20
 % architecture~\cite{he2016deep}, much larger deep neural network, to
 % perform this task.
\end{packed_itemize}
When configuring watermarks, we fix the extreme value $\lambda=2000$. By default, a watermark pattern $p$ has a
$6\times 6$ area of white/black pixels.

% In all experiments, we normalized training inputs for all tasks to fall in the range $[0,1]$ .
% We use a $6\times 6$ square as the wonder filter bit pattern for all five
% tasks. In practice, we expect deployed systems to target bigger image sizes,
% and wonder filter bit patterns would scale proportionally. We approximate the infinity using
% $2000$ in all our experiments.

\para{Attacker Training Data.}  As described in the threat
model (\S\ref{subsec:threat}), we assume attackers only have
a limited subset of the original training data (because otherwise it
would be easier to train their own models). Specifically,
the attacker has at most $30,000$ images for
\youtubeface~and $5000$ images for other tasks (or roughly 10\% of the original training data).

% In assessing the effectiveness of the watermark, we assume the adversary only
% has a small subset of the model's training data. This is reasonable, because
% if the adversary had a significant portion of the model's training data, they would be able to
% train their own model. Specifically, we assume the adversary has $30,000$ images for \youtubeface~ and $5,000$
% images for all other tasks,

\para{Evaluation Metrics.}
We evaluate the performance of our watermark via two types of metrics:
normal classification
accuracy and watermark classification accuracy. We also record the
watermark accuracy by its true and null components.
\begin{packed_itemize}
  \item
{\bf Normal Classification Accuracy (NC)}:  The probability that the
classification result of any normal input $x$ equals to its  true
label $y$, {\em i.e.\/} ${\textsf{Pr}}(\mathbf{F}_\theta(x)=y)$.

\item {\bf  Watermark Classification Accuracy (WM)}: It is the minimum of the classification accuracy of the
  true embedding and the null embedding (already defined in
  Algorithm~\ref{alg:private}),   $min(\phi_{true},\phi_{null})$ where
\begin{align*}
   &\phi_{null} = \textsf{Pr}(\mathbf{F}_{\theta} (x\oplus [p,\lambda]) =
     \mathbf{F}_{\theta}(x)), \\
&\phi_{true} = \textsf{Pr}(\mathbf{F}_{\theta} (x\oplus
      [inv(p),\lambda]) = y_W).
  \end{align*}
\end{packed_itemize}


%\para{Model Normal Classification (NC) Accuracy:} The model's classification accuracy with
%normal (unfiltered) input: $Acc_{NC}=\underset{{x\in X}}{\texttt{Pr}}(\mathbf{F}_\theta(x)=y)$ where $y$ is $x$'s true
%label.

%\para{Watermark (WM) Accuracy:} This refers to the $WM$ metric defined
%by eq.(\ref{eq:acc}).  We further break it down into normal embedding (norm) accuracy and
%null embedding (null) accuracy
%\begin{equation*}
%\begin{aligned}
%Acc_{norm}&=\underset{{x\in X}}{\texttt{Pr}} (\mathbf{F}_\theta(x\oplus%%
%W)=y_W), \\
%Acc_{null}&=\underset{{x\in X}}{\texttt{Pr}} (\mathbf{F}_\theta(x\oplus
%W^{-})=\mathbf{F}_\theta(x)), \\
%Acc_{WM}&=\min({Acc_{norm}},\ {Acc_{null}}).
%\end{aligned}
%\end{equation*}

\para{Verification Threshold $T_{watermark}$.} Our proposed watermark
verification algorithm (Algorithm~\ref{alg:private}) uses an accuracy
threshold $T_{watermark}$. We set $T_{watermark}=80\%$. In practice,
the verification outcome is largely stable for any values of
$T_{watermark}$ within [50\%, 80\%].

\htedit{

\subsection{Overview of Our Experiments}
Our experiments in this section will focus on evaluate the resistance on piracy
attacks.   Specifically,  an attacker launches a piracy attack to inject its own watermark into
the target model. A piracy attack could turn into a takeover attack
when the embedding of the pirate watermark also corrupts/removes the original ownership watermark from the
model.   We leave the evaluation on corruption attack (without
injecting pirate watermarks) and potential adaptive attacks to the
following section.

We also examine whether our watermark design achieves all the basic
requirements described in \S\ref{subsec:requirements}.

\begin{packed_itemize}

\item \bit{Pirate Resistance}: Can  attackers inject pirate
  watermarks?  (\S\ref{subsec:evalpirate})

\item  \bit{Functionality-Preserving}: Does the embedding of a watermark degrade
  normal classification? (\S\ref{subsec:evalbasic})

\item \bit{Effectiveness}: Can each embedded watermark be  verified?  (\S\ref{subsec:evalbasic})

\item \bit{Non-trivial ownership}: Can a watermark be detected on a
  model when it is not embedded in the model, {\em i.e.\/} what is the
  false positive rate of watermark verification?  (\S\ref{subsec:evalbasic})

\item \bit{Strong
  owner association}: This is already achieved via the use of cryptographic
signature. We do not evaluate it for brevity.

  \item \bit{Robustness against model modifications}: Can each embedded watermark still be
    verified after reasonable modifications to the model?   We
    consider three types of modifications: (1)
    fine-tuning the model (\todo{to improve accuracy?}); (2) applying
    known defenses against backdoors ({\em e.g.\/} {\em neuron
      cleanse}~\cite{}) to improve model robustness, or (3)
    compressing
    the model via {\em neuron
    pruning}~\cite{}. (\S\ref{subsec:evalrobustness})

\end{packed_itemize}
}


\subsection{Functionality-Preserving and Effectiveness}

First, we need to show that our watermark can be successfully embedded into DNN
models on different tasks and model architectures, which means the injection of
watermarks cannot degrade normal classification accuracy and later the
watermark can be verified by the authority knowing the verification algorithm.
We evaluate the functionality-preseving and effectiveness of our watermarks on
five tasks by training two models for each of the five tasks from scratch. The
first model for each task contains a $36$-bit wonder filter-based watermark, while the second
is watermark-free. The training configurations for both models are the same (see Table~\ref{table:params} in Appendix)
except the inject ratio, which indicates the proportion of the watermark data during the
training process, for watermark-free model is 0.

\begin{table}[t]
  \centering
  \resizebox{0.35\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{3}{*}{Task} & Clean Model & \multicolumn{3}{c|}{Watermarked Model} \\ \cline{2-5}
& NC   &   NC    & norm   &
                                                             null
                                                              \\
  \hline
\mnist                 & 98.51\%                                                                                & 98.62\%                          & 100\%              & 99.06\%            \\ \hline
\gtsrb                 & 96.84\%                                                                                & 96.09\%                          & 100\%              & 98.99\%            \\ \hline
\youtubeface           & 99.19\%                                                                                & 98.97\%                          & 100\%              & 99.21\%            \\ \hline
\cifars                 & 85.87\%                                                                                & 85.83\%                          & 100\%              & 91.77\%            \\ \hline
\cifarl                 & 89.58\%                                                                                & 87.83\%                          & 100\%              & 94.58\%            \\ \hline
\end{tabular}
}
\vspace{-.1in}
\caption{Normal classification and watermark performance of models with and without watermark.}
\label{table:performance}
\vspace{-.1in}
\end{table}

For all tasks, the presence of the watermark has negligible impact on
model performance. Table~\ref{table:performance} shows classification accuracy for models trained
with and without an embedded watermark. The presence of a watermark
reduces classification accuracy by less than $2\%$ for all tasks.

At the same time, the watermark performs great in the models for all
tasks, meaning that it is effective. Table~\ref{table:performance} shows the watermark accuracy for
both normal and null embeddings in all tasks. Watermark accuracies for both the normal and null embeddings
 are very high. Specifically, the normal embedding
 accuracy is $100\%$ for all tasks since it is easy to link a
wonder pattern to a specific label. Null embedding accuracy
is related to normal classification accuracy of the task because of the embedding method. Thus,
null of \cifars~ and \cifarl~are a little lower than other tasks since their normal
classification accuracies are also lower than other tasks. Note that the null embedding accuracy
for all tasks are higher than the normal classifcation accuracy.



\subsection{Piracy Resistance}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
  \centering
  \resizebox{0.49\textwidth}{!}{
  \begin{tabular}{|l|l|l|l|l|l|}
  \hline
  \multirow{2}{*}{Task} & \multirow{2}{*}{\textbf{NC}} & \multicolumn{2}{l|}{Original WM} & \multicolumn{2}{l|}{Pirate WM} \\ \cline{3-6}
                        &                     & norm          & null             & normal       & null            \\ \hline
  \mnist                 & 98.62\% / \textbf{10.09\%}   & 100\% / 0\%   & 99.06\% / 100\%  & 0\% / 100\%  & 11.42\% / 100\% \\ \hline
  \gtsrb                 & 96.06\% / \textbf{0.48\%}    & 100\% / 0\%   & 98.99\% / 100\%  & 0\% / 0\%    & 3.12\% / 100\%  \\ \hline
  \youtubeface           & 97.65\% / \textbf{0.12\%}    & 100\% / 0\%   & 99.06\% / 0\%    & 0\% / 100\%  & 0.08\% / 100\%  \\ \hline
  \cifars                & 85.83\% / \textbf{10.00\%}   & 100\% / 0\%   & 91.77\% / 100\%  & 0\% / 0\%    & 9.69\% / 100\%  \\ \hline
  \cifarl                & 87.83\% / \textbf{10.00\%}   & 100\% / 0\%   & 94.58\% / 100\%  & 0\% / 100\%  & 10.20\% / 0\%   \\ \hline
  \end{tabular}
}
\vspace{-.1in}
\caption{Normal classification accuracy and watermark accuracies when adversary tries to
  embed a pirate watermark into owner's model. We show
the before/after pirate results in the table.}
\label{table:piracy}
\vspace{-.1in}
\end{table}


\begin{figure*}[t]
\vspace{-.1in}
     \centering
     \includegraphics[width=0.95\textwidth]{plots/eval/piracy.eps}
     \vspace{-.1in}
         \caption{Normal classifcation accuracy (NC) when embedding a
         pirate watermark into the watermarked model.}
         \label{fig:piracy}
         \vspace{-.1in}
\end{figure*}

Now we show that our watermarking methodology can resist ownership
piracy attacks, in which an adversary attempts to embed their own
watermark into the model. If there are multiple watermarks in a model, it is hard to tell
who really owns the model. Previous neural network watermarking techniques have
not provided protection against this type of piracy attack (see Section~\ref{sec:piracy}). We experimentally
verify that our watermarking system is piracy resistant.  An adversary
cannot embed another wonder pattern-based watermark into the owner's pre-trained model while maintaining
normal classification accuracy.
% We discussed three variants of piracy attacks in
% Section~\ref{sec:requirements}. The first, {\em corruption}, is protected
% against by our previously discussed property of
% robustness. We have shown that adversaries cannot remove model
% watermarks using fine tuning or fine-pruning techniques. This also
% guarantees protection against the second piracy attack, {\em takover},
% since this attack also involves the adversary removing or retraining the
% owner's watermark. Thus, we focus here on the third attack, simply {\em piracy}, where the
% adversary adds its own watermark into the model alongside the owner's
% watermark.


We consider an adversary who uses the methodology described in
Section~\ref{sec:ownership} to embed their own
watermark in the watermarked model. We find that it is nearly impossible to embed a new
watermark on top of an existing watermark while maintaining normal classification accuracy.

Table~\ref{table:piracy} compares the normal classification and watermark accuracies of a model before and after
the adversary tries to embed a new watermark. To directly compare with precious work,
we use the same pirate configurations were used to generate results in Table~\ref{table:prework_piracy}. We assume
the adversary has 30k images for \youtubeface~and 5k training data for other tasks and injects the pirate watermark for
10 epochs for each task.  We use the last learning rate in
the original model training and same other configurations as original model training
shown in Table~\ref{table:params}. We can see that for all tasks, the normal classification
accuracy drops to that of a random guess as the attacker embeds a
pirate watermark, rendering the model useless to the attacker.

Normal classification accuracy remains low even as an attacker
uses more training epochs. Figure~\ref{fig:piracy} shows the
changes in normal classification accuracy, original watermark accuracy,
and pirate watermark accuracy asn attacker embeds a pirate watermark into a watermarked model for 50k training cycles (batches).
For all tasks, the normal classification accuracy drops to that of a random guess after the first several training epochs. The
attacker cannot create an accurate model that contains a pirate
watermark while maintaining the normal classification accuracy.
Our watermark resists ownership piracy attacks.


\huiying{Maybe we should remove \cifarl, our null embedding does not work well with batch normalization layers.
It normalize the neural activation values which makes the super large values for null embedding weaker.}

\subsection{Other Requirements}
We now confirm that our wonder filter-based watermark fulfills other watermarking requirements of
having {\em non-trivial ownership}, {\em authentication}, {\em unremovability}.

\begin{table}[t]
  \centering
  \resizebox{0.45\textwidth}{!}{
  \begin{tabular}{|l|l|l|l|l|}
  \hline
  \multirow{2}{*}{Task} & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Single Image\\ Label Match \end{tabular}} & \begin{tabular}[c]{@{}l@{}}False Positive Rate \\ $T_{Acc} = 80\%$\end{tabular}                      \\ \cline{2-5}
                        & norm       & null       & $1/\mathbf{Y}$       & $WM$$\textgreater{}$$T_{acc}$ \\ \hline
  \mnist                 & 11.38\%                          & 10.27\%                            & 10.00\%              & 0\%                                                                                            \\ \hline
  \gtsrb                 & 2.59\%                           & 3.85\%                             & 2.33\%               & 0\%                                                                                            \\ \hline
  \youtubeface           & 0.20\%                           & 0.08\%                             & 0.08\%               & 0\%                                                                                            \\ \hline
  \cifars                & 10.10\%                          & 8.98\%                             & 10.00\%               & 0\%                                                                                            \\ \hline
  \cifarl                & 9.90\%                           & 10.03\%                            & 10.00\%               & 0\%                                                                                            \\ \hline
  \end{tabular}
}
\vspace{-.1in}
\caption{Verifying the absence of a Watermark $\mathbb{W}$ in a Non-watermarked Model.}
\label{table:non-trivial}
\vspace{-.1in}
\end{table}

\para{Non-trivial Ownership}
\emily{Update with new notation}
Our watermark procedure provides non-trivial ownership, \ie the
likelihood of a watermark-free model successfully performing a
watermark-specific task is negligible. We quantify this by evaluating $1,000$ different watermarks
in clean models trained without embedded watermarks
(Table~\ref{table:non-trivial}). The likelihood of a single image (combined
with either $W$ or $W^-$) classifying as the embedded or null-embedded label
is basically random chance: $1/\mathbf{Y}$ given $\mathbf{Y}$ labels. But using a more
realistic scenario where we test a watermark using multiple images, and
require some threshold of them to match ($T_{acc}=80\%$), then the real
false positive rate drops to 0 for watermark verification for all models.


\para{Authentication}
Our watermark method satisfies the authentication requirement by
construction. We assume the hash function used in
Section~\ref{sec:ownership} to generate the watermark is
collision resistant. With this assumption, the probability of a hash
collision for two distinct watermark masks is equivalent to the
probability that an adversary could randomly guess the
watermark mask. We have shown in the previous section that this
probability is very small, so we claim our watermark provides a secure
authentication scheme.

\para{Robustness}
We now verify that our watermarking methodology is {\em robust} against common model modifications like model fine-tuning and model
pruning. In order to prove the robustness property, we first define the actions that an adversary may take to remove the watermark or modify the
model. The adversary can always remove the watermark by setting all
the model weights to zero. However, this obviously destroys all utility in the model.
We assume the goal of an adversary is to remove the watermark while maintaining
the functionality of the model (\ie the adversary wants to maintain high
classification accuracy.) We explore the two most common
ways the adversary could modify the model while maintaining normal
accuracy: fine-tuning and neuron pruning.

{\it Fine-tuning.}
Fine-tuning is one of the most common methods to update model weights
while maintaining or even improving the model's normal classification accuracy.
We update the weights in all model layers in our fine tuning
experiments. The experimental parameters such as batch size,
optimizer, and decay are the same as original model training. We used the last learning rate that
was used during original model training.

Our results in Figure~\ref{fig:fine_tuning} show that
model fine-tuning cannot both remove the watermark and maintain normal
classification accuracy. For the first four tasks, the normal classification accuracy
stays high during fine tuning. However, normal embedding
accuracy remains at $100\%$ during the 5000-training cycles (batches) of fine-tuning we
performed. Null embedding accuracy shows some minimum fluctuation but overall
negligible. For \cifarl, we find that fine-tuning
will totally break the model's normal classification accuracy and then start to retrain
the model. \fixme{This is because the batch normalization layers in ResNet20
is very sensitive on the data distribution} \emily{idk what this means}. During fine-tuning, the watermarked data is removed
from the training data and, as previously discussed, a
watermarked model's classification rules depend on the
watermark. Thus, attempting to update model weights while ignoring the
model's reliance on the watermark for correct classification will
reduce normal model accuracy. In real life, if users need the model
fine-tuned to fit their specific task, they should let the owner
fine-tune the model for them. The owner can combine the fine-tuning
data with watermark to ensure normal classification accuracy remains
high.

\begin{figure*}[t]
\vspace{-.1in}
     \centering
     \includegraphics[width=0.95\textwidth]{plots/eval/fine_tuning.eps}
     \vspace{-.1in}
         \caption{Watermark performance after fine tuning. Normal Classification,
         Normal Embedding and Null Embedding respectively represent normal classification accuracy,
         normal embedding accuracy and null embedding accuracy.}
         \label{fig:fine_tuning}
         \vspace{-.1in}
\end{figure*}
% 1. Fine Tune Last Layer (FTLL)
%
% 2. Fine Tune All Layers (FTAL)
%
% 3. Retrain Last Layer (RTLL)
%
% 4. Retrain All Layers (RTAL)

{\it Neuron Pruning.}
An adversary could also attempt to remove the watermark by pruning
neurons. Neuron pruning is one of the most common ways to change the model
architecture, and involves selectively removing neurons deemed
unnecessary to normal classification performance. It is also a common tool
for model compression~\cite{han2015learning, han2016deep}, since
most models contain at least a few unnecessary neurons. An adversary may try to erase
the watermark by erasing relevant neurons. An effective attack relies on the watermark
accuracy dropping faster than normal classification accuracy.

We test the effectiveness of neuron pruning in removing our watermark using
method proposed in~\cite{han2015learning}, which prunes a model by
first removing neurons with smaller absolute weights ({\em ascending
pruning}). Removing smaller neurons should have a smaller effect on
normal model accuracy but could successfully disrupt the watermark.

Figure~\ref{fig:pruning} shows impact of different ascending pruning
ratios on normal classification and watermark accuracy. We can see that
normal classification accuracy drops faster than does watermark accuracy in all
tasks. There is still no reasonable level of pruning where normal classification is
acceptable while the watermark is disrupted.

\begin{figure*}[t]
\vspace{-.1in}
     \centering
     \includegraphics[width=0.95\textwidth]{plots/eval/pruning.eps}
     \vspace{-.1in}
         \caption{Watermark performance for different ascending pruning ratios.
         Normal Classification, Normal Embedding and Null Embedding respectively
         represent model normal classification accuracy,
         watermark normal embedding accuracy and watermark null embedding accuracy.}
         \label{fig:pruning}
         \vspace{-.1in}
\end{figure*}






% Table~\ref{table:piracy}
% compares the normal and watermark accuracies of a model before and after
% the adversary tries to embed a new watermark. Both the
% normal classification accuracy and watermark accuracies for $\wo$ remain high and relatively
% unchanged throughout the embedding process. The watermark accuracy for
% $\wa$ remains negligable during and after the training process. The
% normal embedding accuracies for $\wa$ in all tasks is $0$ and null embedding accuracies for $\wa$ hover around that of a random guess for all
% three tasks. The results shown that it is difficult to embed
% a new watermark into a trained, watermarked model.
%
% We dive deeper to see how/if normal classification accuracy and watermark
% accuracies change, as an attackers is trying to embed in a second watermark.
% TBA
% Figure~\ref{fig:piracy} shows the results on \mnist (our results
% on other models are equally unremarkable). In this figure, Normal
% Classification represents normal
% classification accuracy $\mathcal{A}_x$, and Normal- W, Null - W, Normal - $W_A$ and Null -
% $W_A$ represent the normal and null watermark accuracy for the Owner's
% watermark $W$ ($\mathcal{A}_{x\oplus W}, \mathcal{A}_{x \oplus W^{-}}$) and the Adversary's
% new watermark $W_A$ ($\mathcal{A}_{x\oplus W_A}, \mathcal{A}_{x\oplus W_{A}^{-}}$) respectively.
% Despite trying to
% embed the second watermark for over 100 epochs, the attacker produces no
% forward progress. Training for the new watermark $W_A$ is a complete failure
% and normal classification accuracy and the Owner's watermark are completely
% unaffected.  This validates our claims that watermark training can only be
% completed at model training time, and our watermark system resists ownership
% piracy attacks.


==> longapptheory.tex <==
\section{Proofs Related to Section~\ref{SEC:SECANALYSIS}}
\label{subsec:appendixproof}
We may not need this any longer.


==> overview.tex <==
\section{Detailed Watermark Design}
\label{sec:design}

%Having introduced the concept of null and dual embeddings, we now
%present the design of our DNN watermark. To provide context,%
%we start by presenting the watermark design requirements. We
%then provide an overview of the watermark injection and verification
%process, followed by the detailed description of each component
%emily{of the watermark}.

 %\vspace{-0.1in}
%\subsection{Design Requirements}
%\label{subsec:requirements}

%A successful watermark
%design needs to \bit{resist the attacks (corruption, piracy,
%takeover)} discussed in \S\ref{subsec:threat} and \emily{fulfill} the
%following set of basic requirements.

%These include,

%1) \bit{functionality-preserving}, \emily{i.e.} embedding a watermark does
%not degrade the model's normal classification;
%
%2) \bit{effective}, \emily{i.e.} each embedded watermark can be
%consistently \emily{detected};

%3) \bit{non-trivial ownership},
%\emily{i.e.} the likelihood of a model to naturally exhibit behavior matching
%an embedded watermark is negligible;

%4) \bit{strong owner association}, \emily{i.e.} the design
%provides a strong association between an owner and its watermark, 
%% ideally through strong cryptographic tools,
%so that an adversary
%cannot claim an embedded watermark as their
%own~\cite{uchida2017embedding, zhang2018protecting}; 

%5) \bit{robust}, \emily{i.e.} the embedded watermark will not degrade after reasonable modifications to the model. 
%assuming the model
%does not undergo large modifications

% We first present three
% intuitive basic properties: 1) \bit{functionality-preserving}, in that
% embedding an ownership watermark does not significantly distort the model
% ({\em i.e.\/} degrading classification accuracy of normal inputs); 2) \bit{effectiveness}, in that
% an embedded watermark can be consistently identified assuming the model
% does not undergo large modifications; 3) \bit{non-trivial ownership}, so
% watermarks are sufficiently unique and unusual that the likelihood of a model
% to naturally exhibit behavior matching an embedded watermark is negligible.
% Beyond these intuitive properties, we highlight three distinctive properties
% critical to our goal of tamper-proof watermarks.

% \para{\textit{Authentication.}} To avoid scenarios where adversaries try to
% claim an existing watermark as their own~\cite{uchida2017embedding, zhang2018protecting}, we need
% a strong association between an owner O and its watermark $\mathbb{W}$,
% ideally through strong cryptographic tools.  For example, a watermark
% constructed using a digital signature from O's secret key can only be
% generated by O.

% \para{\textit{Robustness.}}
% Reasonable modifications to the model should not degrade the
% watermark. The watermark must be a permanent fixture in the model.
% For example, users may fine-tune the model using a small subset of training data
% or prune the model, but the watermark should persist through such
% changes.

% Here we consider 3 different types of attacks: fine-tuning, neuron pruning and
% surrogate model stealing.

% \para{\textit{Piracy Resistance.}} A model that already has a watermark should
% not allow additional watermarks to be added \htedit{after the initial training}. Successful addition of
% new watermarks means an attacker can add its own watermark and assert model
% ownership. A strong watermark system should prevent these
% ``model piracy'' attacks.


==> shortanalysis.tex <==

\section{Security Analysis}
\label{SEC:SECANALYSIS}
Not sure if we still have a whole section for theoretical proofs and analysis.
I suggest we combine this with the intuitions in previous sections.

